Practical and Fast Momentum-Based Power Methods

The power method is a classical algorithm with broad applications in machine learning tasks, including streaming PCA, spectral clustering, and low-rank matrix approximation. The distilled purpose of the vanilla power method is to determine the largest eigenvalue (in absolute modulus) and its eigenvector of a matrix. A momentum-based scheme can be used to accelerate the power method, but achieving an optimal convergence rate with existing algorithms critically relies on additional spectral information that is unavailable at run-time, and sub-optimal initializations can result in divergence. In this paper, we provide a pair of novel momentum-based power methods, which we call the delayed momentum power method (DMPower) and a streaming variant, the delayed momentum streaming method (DMStream). Our methods leverage inexact deflation and are capable of achieving near-optimal convergence with far less restrictive hyperparameter requirements. We provide convergence analyses for both algorithms through the lens of perturbation theory. Further, we experimentally demonstrate that DMPower routinely outperforms the vanilla power method and that both algorithms match the convergence speed of an oracle running existing accelerated methods with perfect spectral knowledge.

==> algos/algo2-PAPM.tex <==

\begin{algorithm}[!ht]
    \caption{Partially Adaptive Power Method (PAPM)}
    \label{alg:papm}
\begin{algorithmic}[1]
\Require $A\in\mathbb{R}^{d\times d}$ symmetric, unit $q_0\in\mathbb{R}^d$, unit $w_0\in\mathbb{R}^d$, $\epsilon<1$, $\rho<1$ 
\Ensure $\epsilon$-accurate approximation $q_k$ of $v_1$, i.e., $1-(q_k^{\top}v_1)^2<\epsilon$
\State $q_{-1} = \textbf{0}$
\State $\nu_1\leftarrow q_0^{\top}Aq_0$
\State $\beta_1\leftarrow \nu_1$ \Comment Initial momentum coefficient
\For{$k=2,3,\dots$} \Comment{while $\left\lVert q_{k}-q_{k-1}\right\rVert > \epsilon$}
\State $q_{k} \leftarrow Aq_{k-1} -\beta_{k}q_{k-2}$
\State $q_{} \leftarrow q_{k}/\norm{q_{k}}$
\State $\nu_k \leftarrow q_{k}^{\top}Aq_{k}$ \Comment{Rayleigh Quotient estimate of $\lambda_1$}
\If {$|\lambda_2-\mu_{k}|>\rho$}
    \State $P\leftarrow \nu_{k}q_kq_k^{\top}$
    \State $w_k\leftarrow(A-P)w_{k-1}$ \Comment{Inexact deflation}
    \State $w_k \leftarrow w_k/\norm{w_k}$
    \State $\mu^{(k)} \leftarrow w_k^{\top}Aw_k$ \Comment{Rayleigh Quotient estimate of $\lambda_2$}
    \State $\beta_k \leftarrow \mu_k^2/4$ \Comment{Approximated optimal momentum coefficient}
\Else
\State $\beta_k \leftarrow \beta_{k-1}$ \Comment{Do not update $\beta_k$ anymore}
\EndIf
\EndFor
\Return{$q_k,\nu_k$} 
\end{algorithmic}
\end{algorithm}


% \begin{algorithm}[!ht]
% \caption{Partially-Adaptive Momentum Power Method {\color{blue}[AR: REVISED]}}
% \label{alg:papm}
% \begin{algorithmic}
% \Require $A\in\mathbb{R}^{n\times n}$ diagonalizable, initial vector $\vec{q}^{(0)}\in\mathbb{R}^n$ for primary power method, $\vec{q}^{(-1)}=\textbf{0}$, error threshold for $\vec{x}_1$ estimate $\epsilon$, error threshold for $\vec{x_2}$ estimate $\rho$
% \Ensure Dominant eigenvector $\vec{x}_1$, eigenvalue $\lambda_1$
% \State $\vec{w}^{(-1)} = \textbf{0}$
% \State $\vec{w}^{(0)} \leftarrow \vec{q}^{(0)}$
% \For{$k=1,2,\dots$} 
% \Comment{while $\left\lVert \vec{q}^{(k-1)}-\vec{q}^{(k-2)}\right\rVert > \epsilon$}
% \If{$\left\lVert \vec{w}^{(j-1)}-\vec{w}^{(j-2)}\right\rVert > \rho$}
% \State $\vec{z}^{(j)} \leftarrow A\vec{q}^{(j-1)}-\beta^{(j)}\vec{q}^{(j-2)}$ \Comment{obtain optimal momentum coeff. via concurrent iteration \fh{the algorithm pseudo code is off. What is $j$?}}
% \State $\vec{q}^{(j)} \leftarrow \vec{z}^{(j)}/\norm{\vec{z}^{(j}}$
% \State $\lambda^{(j)} \leftarrow (\vec{q}^{(k)})^\textrm{T}A\vec{q}^{(j)}$ \Comment{Rayleigh Quotient estimate of $\lambda_1$}
% \State $P\leftarrow \lambda^{(j)}\vec{q}^{(j)}[\vec{q}^{(j)}]^{\textrm{T}}$
% \State $\vec{y}^{(j)}\leftarrow(A-P)\vec{w}^{(j-1)}$ \Comment{Inexact deflation}
% \State $\vec{w}^{(j)} \leftarrow \vec{y}^{(j)}/\norm{\vec{y}^{(j}}$
% \State $\mu^{(j)} \leftarrow (\vec{w}^{(k)})^\textrm{T}A\vec{w}^{(j)}$ \Comment{Rayleigh Quotient estimate of $\lambda_2$}
% \State $\beta^{(j)}\leftarrow [\mu^{(j)}]^2/4$
% \EndIf
% \State $\beta \leftarrow [\mu^{(j)}]^2/4$ \Comment{Approximated optimal momentum coefficent}
% \State $\vec{q}^{(1)} \leftarrow \vec{q}^{(k)}$  \Comment{Current estimate of $\vec{x}_1$}
% \State $\vec{z}^{(k)} \leftarrow A\vec{q}^{(k-1)}-\beta\vec{q}^{(k-2)}$ \Comment{Momentum update}
% \State $\vec{q}^{(k)} \leftarrow \vec{z}^{(k)}/\norm{\vec{z}^{(k}}$
% \State $\lambda^{(k)} \leftarrow (\vec{q}^{(k)})^\textrm{T}A\vec{q}^{(k)}$
% \EndFor
% \Return{$\vec{q}^{(k)},\lambda^{(k)}$} 
% \end{algorithmic}
% \end{algorithm}

==> manuscript/RhoVarianceExperiment-LooseEigengaps.tex <==
% This file was created by tikzplotlib v0.9.2.
\begin{tikzpicture}[scale=0.54]

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{1,0.498039215686275,0.0549019607843137}
\definecolor{color2}{rgb}{0.172549019607843,0.627450980392157,0.172549019607843}
%red
\definecolor{color3}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}
%purple
\definecolor{color4}{rgb}{0.580392156862745,0.403921568627451,0.741176470588235}
%brown
\definecolor{color5}{rgb}{0.549019607843137,0.337254901960784,0.294117647058824}

\begin{axis}[
legend cell align={left},
legend style={nodes={scale=0.7, transform shape}, fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
log basis x={10},
tick align=outside,
tick pos=left,
title={{Loose Eigengaps: \texttt{spec}=[1, 0.9, 0.8,\dots, 0.8]}},
x grid style={white!69.0196078431373!black},
xlabel={Error Threshold},
xmajorgrids,
xmin=5.01187233627271e-09, xmax=0.0199526231496888,
xmode=log,
xtick style={color=black},
y grid style={white!69.0196078431373!black},
ylabel={Iteration Count},
ymajorgrids,
ymin=0, ymax=85,
ytick style={color=black}
]
\addplot [color0, dashed, mark=diamond*, mark size=2.5, mark options={solid}]
table {%
1e-08 80.768
1e-07 70.053
1e-06 58.549
1e-05 48.201
0.0001 37.39
0.001 27.131
0.01 16.787
};
\addlegendentry{Vanilla Power Method}
\addplot [color1, dashed, mark=asterisk, mark size=2.5, mark options={solid}]
table {%
1e-08 34.603
1e-07 29.647
1e-06 26.136
1e-05 21.484
0.0001 17.693
0.001 13.377
0.01 9.344
};
\addlegendentry{Power + M, $\beta=0.2025$}
\addplot [color2, mark=triangle*, mark size=2.5, mark options={solid}]
table {%
1e-08 66.482
1e-07 58.16
1e-06 49.857
1e-05 41.59
0.0001 33.323
0.001 23.722
0.01 13.192
};
\addlegendentry{DMPM, $\rho = \epsilon$}
\addplot [color3, mark=triangle*, mark size=2.5, mark options={solid}]
table {%
1e-08 57.138
1e-07 49.859
1e-06 41.765
1e-05 33.91
0.0001 25.079
0.001 17.761
0.01 12.204
};
\addlegendentry{DMPM, $\rho = \sqrt{\epsilon}$}
\addplot [color4, mark=triangle*, mark size=2.5, mark options={solid}]
table {%
1e-08 53.907
1e-07 45.606
1e-06 36.368
1e-05 28.915
0.0001 22.91
0.001 17.77
0.01 12.127
};
\addlegendentry{DMPM, $\rho = \sqrt[3]{\epsilon}$}
\addplot [color5, mark=triangle*, mark size=2.5, mark options={solid}]
table {%
1e-08 48.979
1e-07 41.162
1e-06 33.505
1e-05 28.334
0.0001 22.977
0.001 17.833
0.01 12.077
};
\addlegendentry{DMPM, $\rho = \sqrt[4]{\epsilon}$}
\end{axis}

\end{tikzpicture}


==> manuscript/RhoVarianceExperiment-MedEigengaps.tex <==
% This file was created by tikzplotlib v0.9.2.
\begin{comment}
\begin{tikzpicture}[scale=.54]

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{1,0.498039215686275,0.0549019607843137}
\definecolor{color2}{rgb}{0.172549019607843,0.627450980392157,0.172549019607843}
\definecolor{color3}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}
\definecolor{color4}{rgb}{0.580392156862745,0.403921568627451,0.741176470588235}
\definecolor{color5}{rgb}{0.549019607843137,0.337254901960784,0.294117647058824}

\begin{axis}[
legend cell align={left},
legend style={nodes={scale=0.7, transform shape}, fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
log basis x={10},
tick align=outside,
tick pos=left,
title={Med Eigengaps: \texttt{spec}=[1, 0.99, 0.98,\dots, 0.98]},
x grid style={white!69.0196078431373!black},
xlabel={Error Threshold},
xmajorgrids,
xmin=5.01187233627271e-09, xmax=0.0199526231496888,
xmode=log,
xtick style={color=black},
y grid style={white!69.0196078431373!black},
ylabel={Iteration Count},
ymajorgrids,
ymin=0, ymax=500,
ytick style={color=black}
]
\addplot [color0, dashed, mark=diamond*, mark size=2.5, mark options={solid}]
table {%
1e-06 238.44
1e-05 203.14
1e-04 157.48
1e-03 107.94
1e-02 75.86
1e-01 2.0
};
\addlegendentry{DMPM, $\rho = \sqrt{\epsilon}$}

\addplot [color1, dashed, mark=diamond*, mark size=2.5, mark options={solid}]
table {%
1e-06 252.7
1e-05 196.44
1e-04 152.34
1e-03 124.94
1e-02 73.98
1e-01 2.0
};
\addlegendentry{DMPM, $\rho = \sqrt[3]{\epsilon}$}

\addplot [color2, dashed, mark=diamond*, mark size=2.5, mark options={solid}]
table {%
1e-06 245.96
1e-05 197.26
1e-04 162.04
1e-03 115.62
1e-02 83.54
1e-01 2.0
};
\addlegendentry{DMPM, $\rho = \sqrt[4]{\epsilon}$}

\addplot [color3, dashed, mark=diamond*, mark size=2.5, mark options={solid}]
table {%
1e-06 542.9
1e-05 430.52
1e-04 315.66
1e-03 206.52
1e-02 100
1e-01 100
};
\addlegendentry{Lanczos}

\addplot [color4, dashed, mark=diamond*, mark size=2.5, mark options={solid}]
table {%
1e-06 258.5
1e-05 195.94
1e-04 152.92
1e-03 122.02
1e-02 78.96
1e-01 2.0
};
\addlegendentry{DMPM, $\rho = \epsilon$}

\addplot [color5, dashed, mark=diamond*, mark size=2.5, mark options={solid}]
table {%
1e-06 503.3
1e-05 387.58
1e-04 276.8
1e-03 240.32
1e-02 142.22
1e-01 1.0
};
\addlegendentry{Power Method}

\addplot [color6, dashed, mark=diamond*, mark size=2.5, mark options={solid}]
table {%
1e-06 238.94
1e-05 190.06
1e-04 151.44
1e-03 118.94
1e-02 71.52
1e-01 1.0
};
\addlegendentry{Power + M Method}
\end{axis}

\end{tikzpicture}
\end{comment}


==> manuscript/RhoVarianceExperiment-TightEigengaps.tex <==
% This file was created by tikzplotlib v0.9.2.
\begin{tikzpicture}[scale=0.54]

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{1,0.498039215686275,0.0549019607843137}
\definecolor{color2}{rgb}{0.172549019607843,0.627450980392157,0.172549019607843}
\definecolor{color3}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}
\definecolor{color4}{rgb}{0.580392156862745,0.403921568627451,0.741176470588235}
\definecolor{color5}{rgb}{0.549019607843137,0.337254901960784,0.294117647058824}
\definecolor{color6}{rgb}{0.459019607843137,0.287254901960784,0.214117647058824}

\begin{axis}[
legend cell align={left},
legend style={nodes={scale=0.7, transform shape}, fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
log basis x={10},
tick align=outside,
tick pos=left,
title={Tight Eigengaps: \texttt{spec}=[1, 0.999, 0.998,\dots, 0.998]},
x grid style={white!69.0196078431373!black},
xlabel={Error Threshold},
xmajorgrids,
xmin=5.01187233627271e-07, xmax=0.0199526231496888,
xmode=log,
xtick style={color=black},
y grid style={white!69.0196078431373!black},
ylabel={Iteration Count},
ymajorgrids,
ymin=0, ymax=4000,
ytick style={color=black}
]
\addplot [color0, dashed, mark=diamond*, mark size=2.5, mark options={solid}]
table {%
1e-06 1967.6
1e-05 1486.5
1e-04 1071.12
1e-03 748.98
1e-02 2.0
1e-01 2.0
};
\addlegendentry{DMPM, $\rho = \sqrt{\epsilon}$}

\addplot [color1, dashed, mark=diamond*, mark size=2.5, mark options={solid}]
table {%
1e-06 2006.6
1e-05 1494.56
1e-04 1209.58
1e-03 760.48
1e-02 2.0
1e-01 2.0
};
\addlegendentry{DMPM, $\rho = \sqrt[3]{\epsilon}$}
\addplot [color2, dashed, mark=diamond*, mark size=2.5, mark options={solid}]
table {%
1e-06 2002.58
1e-05 1526.08
1e-04 1081.86
1e-03 764.96
1e-02 2.0
1e-01 2.0
};
\addlegendentry{DMPM, $\rho = \sqrt[4]{\epsilon}$}
\addplot [color3, dashed, mark=diamond*, mark size=2.5, mark options={solid}]
table {%
1e-06 3434.32
1e-05 2245.16
1e-04 1164.24
1e-03 100.0
1e-02 100.0
1e-01 100.0
};
\addlegendentry{Lanczos}
\addplot [color4, dashed, mark=diamond*, mark size=2.5, mark options={solid}]
table {%
1e-06 1989.62
1e-05 1458.9
1e-04 1136.22
1e-03 685.56
1e-02 2.0
1e-01 2.0
};
\addlegendentry{DMPM, $\rho = \epsilon$}
\addplot [color5, dashed, mark=diamond*, mark size=2.5, mark options={solid}]
table {%
1e-06 4013.02
1e-05 2943.5
1e-04 2232.3
1e-03 1431.5
1e-02 1.0
1e-01 1.0
};
\addlegendentry{Power Method}
\addplot [color6, dashed, mark=diamond*, mark size=2.5, mark options={solid}]
table {%
1e-06 2002.02
1e-05 1433.3
1e-04 1169.3
1e-03 690.08
1e-02 1.0
1e-01 1.0
};
\addlegendentry{Power + M Method}
\end{axis}

\end{tikzpicture}

